Assessing differentially private deep learning with Membership Inference

Attacks that aim to identify the training data of public neural networks represent a severe threat to the privacy of individuals participating in the training data set. A possible protection is offered by anonymization of the training data or training function with differential privacy. However, data scientists can choose between local and central differential privacy and need to select meaningful privacy parameters $\epsilon$ which is challenging for non-privacy experts. We empirically compare local and central differential privacy mechanisms under white- and black-box membership inference to evaluate their relative privacy-accuracy trade-offs. We experiment with several datasets and show that this trade-off is similar for both types of mechanisms. This suggests that local differential privacy is a sound alternative to central differential privacy for differentially private deep learning, since small $\epsilon$ in central differential privacy and large $\epsilon$ in local differential privacy result in similar membership inference attack risk.

==> defi.tex <==
%%custom packages
% Magic hack for subcaption and svg compatibility
% https://tex.stackexchange.com/questions/291929/svg-package-and-subcaption-incompability
\RequirePackage{scrlfile}
\PreventPackageFromLoading{subfig}

\usepackage[inline]{enumitem}
%\usepackage{cite}
\usepackage{todonotes}
\usepackage{csquotes}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{multicol} 
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{subcaption}
\usepackage{graphicx}
\usepackage{hyperref}
%\let\proof\relax
%\let\endproof\relax
%\let\theorem\relax
%\let\endtheorem\relax
%\usepackage{amsthm}
\usepackage{tikz}
\usepackage{pdfpages}
\usepackage{tabularx}
\usepackage{mathrsfs}
\usepackage{amsmath,amssymb,amstext}
%\usepackage{algorithmic}
\usepackage{algorithm}
\usepackage{algpseudocode}

\usetikzlibrary{shapes, fit}

\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}
\algnewcommand\algorithmicoutput{\textbf{Output:}}
\algnewcommand\Output{\item[\algorithmicoutput]}

\usepackage{url}
\usepackage{textcomp}
\usepackage{xcolor}
\graphicspath{{fig/}}
%% Custom definitions
\newcommand{\eps}{\ensuremath{\epsilon}}
\newcommand{\dlt}{\ensuremath{\delta}}
\newcommand{\sgm}{\ensuremath{\sigma}}
\newcommand{\tht}{\ensuremath{\theta}}
\newcommand{\epsdlt}{\ensuremath{(\epsilon,\delta)}}
\newcommand{\money}[1]{\$#1}
\newcommand{\person}[1]{\textsc{#1}}
\newcommand{\cali}[1]{\ensuremath{\mathcal{#1}}} % for uppercase letters only
\newcommand{\var}[1]{\ensuremath{\mathtt{#1}}}
\newcommand{\varbf}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\subscr}[2]{\ensuremath{#1_{\var{#2}}}}
\newcommand{\supscr}[2]{\ensuremath{#1^{\var{#2}}}}
\newcommand{\subsup}[3]{\ensuremath{#1_{\var{#2}}^{\var{#3}}}}
\newcommand{\pprime}{\ensuremath{\prime}}
\newcommand{\filenamename}{\edef\foo{\currfilebase}}
\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{definition}{Definition}

% \newtheoremstyle{defistyle}% name für den Stil

%  {}%      Space above

%  {}%      Space below

%  {\itshape}%      Body font

%  {}%      Indent amount (empty = no indent, \parindent = para indent)

%  {\bfseries\sffamily}% Thm head font

%  {\rm.}%        Punctuation after thm head

%  { }% Space after thm head: " " = normal interword space; \newline = linebreak

%  {} %{\textbf{\thmname{Definition}} (\thmnote{#3})}%         Thm head spec (can be left empty, meaning `normal')

%  % http://www.stat.umn.edu/~charlie/amslatex.html <http://www.stat.umn.edu/~charlie/amslatex.html> 

% \theoremstyle{defistyle}

% quotes

\newcommand{\bq}{``}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\green}[1]{\textcolor{teal}{#1}}
\newcommand{\orange}[1]{\textcolor{orange}{#1}}


\newcommand{\rred}[1]{\textcolor{black}{#1}}

\newcommand{\eq}{''}

\newcommand{\q}[1]{\bq{#1}\eq}

\renewcommand{\vec}[1]{\mathbf{#1}}

\tikzset{
	double color fill/.code 2 args={
		\pgfdeclareverticalshading[%
			tikz@axis@top,tikz@axis@middle,tikz@axis@bottom%
		]{diagonalfill}{100bp}{%
			color(0bp)=(tikz@axis@bottom);
			color(50bp)=(tikz@axis@bottom);
			color(50bp)=(tikz@axis@middle);
			color(50bp)=(tikz@axis@top);
			color(100bp)=(tikz@axis@top)
		}
		\tikzset{shade, left color=#1, right color=#2, shading=diagonalfill}
	}
}


==> src/revision.tex <==
\onecolumn
{
    \hfill \large{Response to Reviewer Comments, \today} \\
       \small
    Dear anonymous reviewers,
    \\[1mm]
    thank you for the opportunity to submit a revision of our work. We provide an overview of our changes per weakness (W) and detailed comment (D) followed by a latexdiff of the paper. We repeated all black-box MI experiments with an adapted methodology that incorporates your feedback and added a new white-box MI attack evaluation. Major changes comprise the use of early stopping in all ML models (target-, shadow-, and attack model) for better generalization and real world relevance, and a novel definition of $\varphi$. Furthermore, taking into account D5 of Reviewer 1 we decided to calculate MI attack performance as the area under the receiver operating curve (i.e., ratio of True Positive Rate to False Positive Rate). The resulting experiments spanned over weeks and we analyzed several terabytes of data. We feel confident in claiming that the changes substantially improved this paper. We plan to provide access to our code and data together with a technical report that also shows graphs and discussions that do not fit into the paper due to length restrictions.
    \\[3mm]
Reviewer 1
\vspace{1pt}
\hrule
\vspace{2pt}  
    \begin{itemize}
%        \item W1: \textit{Methodology has some puzzling choices.} 
%         \begin{itemize}
%         \item We addressed this weakness in our response to your detailed comment D11.
%         \end{itemize}
        \item D1: \textit{It is important to observe that each experiment combines two separate components: (1) a DP algorithm and (2) an membership inference attack algorithm. The accuracy and $\epsilon$ come from (1) but the MI attack success rate comes from the combination of (1) and (2). So for instance, a poorly designed attack algorithm could lead you to erroneously conclude that a particular DP algorithm poses low MI risk. The paper largely ignores this subtlety and ascribes the MI risk as an intrinsic property of the DP algorithm.}\\
%        \item D1: \textit{The paper ascribes the MI risk solely as an intrinsic property of the DP algorithm.}
        \blue{R: We agree with the observation. Membership inference attacks (MIA) can only provide a lower bound on the inference risk while DP provides an upper bound on the inference risk. Yeom et al.~\cite{YGF+18} have demonstrated that the upper bound for CDP can be converted into an expected bound for MIA. However, for DP-SGD the lower and the upper bound lie far away from each other given that relatively large $\epsilon$ already result in low attack precision. Our novel observation is that the lower and the upper bound lie even farther apart from each other for LDP which leads us to conclude that LDP with high $\epsilon$ values is still an alternative to the DP-SGD with smaller $\epsilon$ values. It is furthermore true, that our results depend on the specific MIA that is used. We added a series of white-box MIA results to illustrate how the bounds for DP and MI behave when MIA with stronger assumptions are used.}
        \item D2: \textit{Prior work by Abowd and Schmutte \cite{abowd2019} outlines a methodology for studying privacy-utility trade-offs using the concept of the production possibility frontier. The authors should at the very least cite this paper but also should consider adopting this methodology, particularly the idea of a PPF. Figures i and j come the closest to the Abowd and Schmutte approach.}\\
%        \item D2: \textit{Production Possibility Frontier: Authors should at the very least citePrior work by Abowd and Schmutte.}
        \blue{R: Thank you for this suggestion and indeed we have some similarity to Abowd and Schmutte (e.g., empirically analyzing the production function of $\epsilon$ and accuracy). However, we do not have access to a social welfare function that describes aggregate preferences for the privacy loss and accuracy. If such a function would be available in our scenario it would allow us to identify \eps~at which CDP and LDP meet the socially acceptable privacy-accuracy trade-off. We argue that these $\epsilon$ do not give us enough information about factual protection against MIA. In consequence we empirically determine a second production frontier for MI over \eps~and calculate the relative privacy-accuracy trade-off at both production frontiers for every \eps. This allows data scientists to assess whether losses in accuracy are outweighing gains in privacy, and to compare LDP and CDP mechanisms aside from \eps. We integrated the reference into related work. Furthermore we revised our definition of $\varphi$.}
        \item D3: \textit{The paper omits a privacy-utility comparison using $\epsilon$ as the measure of privacy loss. I think this should be included because it will bring the results into context. For instance, Figures i and j could be replicated but with $\epsilon$ in place of MI attack success rate.}\\
%        \item D3: \textit{The paper omits a privacy-utility comparison using $\epsilon$ as the measure of privacy loss which will bring the results into context. Figures i and j could be replicated but with $\epsilon$ in place of MI attack success rate.}
        \blue{R: Thank you for this suggestion. We added an additional scatterplot over $\epsilon$ to the existing scatterplots over MI AUC in Figure 3 -- 6k. Furthermore, a comparison over $\epsilon$ is depicted in the graphs in Figure (a) and (e) per dataset (MI AUC over $\epsilon$ for CDP/LDP).}
        \item D4: \textit{The range of $\epsilon$ should be large enough to show the full range of algorithm behavior. If we tried CDP with higher $\epsilon$ values, we would presumably see blue dots with higher test accuracy. Would the new blue dots come in above or below the red diamonds?}\\
%        \item D4: \textit{The range of $\epsilon$ should be large enough to show the full range of algorithm behavior.}
        \blue{R: Indeed we missed these areas in the privacy parameter search space. We extended the range of $\epsilon$ values in LDP and CDP to obtain differentially private models between baseline accuracy (i.e., no utility) and almost original accuracy (i.e., full utility).}
        \item D5: \textit{The paper reports precision and recall separately, which may lead to misleading conclusions. Precision and recall are tunable. If my attack model was logistic regression, I could vary the threshold for assigning class labels. Raising the threshold will generally raise precision and lower recall. Generally LDP reports low recall but higher precision. Is this simply because its effective threshold is higher than the one learned for CDP? If we tweaked the threshold a bit would we see different curves? An alternative to consider would be area under the ROC curve, which in a sense captures precision-recall across all possible thresholds.}\\
%        \item D5: \textit{The paper reports precision and recall separately, which may lead to misleading conclusions. Precision and recall are tuneable. If my attack model was logistic regression, I could vary the threshold for assigning class labels. Raising the threshold will generally raise precision and lower recall. Generally LDP reports low recall but higher precision. Is this simply because its effective threshold is higher than the one learned for CDP? If we tweaked the threshold a bit would we see different curves? An alternative to consider would be area under the ROC curve, which in a sense captures precision-recall across all possible thresholds.}   
        \blue{R: We agree with your argument, especially since the MIA represent binary classifiers. In consequence, we decided to replace the individual discussion of MI precision and recall with the ROC area under curve.}
        \item D6: \textit{The $\varphi$ measure is problematic: when the precision of the MI attack under DP is 50\%, the denominator becomes zero, rendering $\varphi$ undefined. The practical value of a relative measure is unclear and the user might prefer low MI precision in absolute terms.}\\
        % \item D6: \textit{$\phi$ measure issues: First, when the precision of the MI attack under \eps-DP is 50\%, the denominator becomes zero, rendering $\phi$ undefined. Practical value of a relative measure is unclear. User might prefer low MI precision in absolute terms.}
         \blue{R: Indeed the denominator of $\varphi$ must not become 0 and the definition of $\varphi$ comprised several shortcomings. Taking also into account other review comments on $\varphi$ we revised our definition of $\varphi$ to reflect the relative decrease in the area under the MI receiver operating characteristics divided by the relative decrease in test accuracy. This revised definition still reflects our motivation to allow weighing gains in privacy against losses in accuracy. The trade-off will only be beneficial for the data owner within a subset of possible privacy parameters. $\varphi$ allows to identify privacy parameters which provide favorable ratios of decreases in MIA risk and test accuracy. For a calculation of the privacy-utility trade-off at a given privacy measure (e.g., MI AUC 80\%) $\varphi$ is not useful, but the data scientist can use a graph like Fig.~(a) or scatterplot like Fig.~(k).}
        \item D7: \textit{Error bars should be presented consistently.}\\
        \blue{R: For all Figures besides the scatter plots error bars are used already. However, for Texas Hospital Stays and Purchases in Figure~3 and~4 the error bars are very narrow and thus lie within the points. We made sure to explicitly mention this in the figure captions.
        In this revision we added Figures with ROC curves (i.e., Figure~(i)). 
        The ROC curves depict the mean linear interpolation of the True Positive Rate over the False Positive Rate of five independent experiment repetitions. Error bars for the mean interpolation of the True Positive Rate would have drastically decreased readability. 
        The scatterplots in Figure 3, 4, 6, 7 (k) depict the AUC of the mean interpolation of the True Positive Rate over all independent experiment runs, instead of the mean AUC score over all independent experiment runs. Thus, we also omitted error bars in these Figures.}
        \item D8: \textit{The authors may want to use results on shuffling to lower the effective $\epsilon$ of their LDP approach.}\\
        \blue{R: Thank you for pointing out this possible optimization for LDP mechanisms. We understand that the use of shuffling would require two parties in order to achieve one advantage of LDP -- security against a central party, one for shuffling and one for analysis. However, we are solely considering one party in this paper (i.e., the data analyst) to ensure a fair comparison of LDP and CDP. We keep multiple parties, as also found in federated learning, as future work and will integrate shuffling there.}
        \item D9: \textit{For several datasets, it looks like fewer classes leads to higher MI attack success. Counter to what was observed in~\cite{shokri2017}.}\\
        \blue{R: This effect is indeed observable w.r.t.~MI recall for Texas Hospital Stays, Purchases, and LFW. However, MI recall has not been considered in the original paper of Shokri et al.~\cite{shokri2017}. They state MI precision, and show that the MI precision increases with more classes in the dataset. We also see this for MI Precision for Texas Hospital Stays, Purchases and LFW. MIA works better for classes with few member records than for classes with many records. The Skewed Purchases dataset is different to the other datasets since it is balanced. Thus, class imbalances leading to more classes with fewer members cannot be exploited by MIA. Instead, the overall train-test gap is the dominant indicator for the MI precision on this dataset instead of the class distribution. The train test gap is higher when all classes have many records (e.g., $\mathbb{C}=10$) than when all classes have a small number of records (e.g., $\mathbb{C}=100$). We added this explanation to Section~\ref{sec:data} and provide plots that support the argument in a technical report.}
        \item D10: \textit{Algorithms are run at vastly different $\epsilon$. There's no meaningful alignment between fig.~a,b,c and d,e,f.}\\
%        \item D10: \textit{Algorithms are run at vastly different epsilons. No meaningful alignment between x-axis of figures a,b,c and d,e,f..}
        \blue{R: We understand that the large difference between the $\epsilon$ values in LDP and CDP can be irritating. However, we show that these vastly different $\epsilon$ values provide comparable protection against MIA and hence scale our graphs to depict this comparison. Due to the differing neighbouring definitions of LDP and CDP, $\epsilon$ values lie on different scales. LDP can transfer any record in a dataset with a bounded probability into any other record from the dataset domain, whereas CDP achieves that every mechanism output could have been produced with a bounded probability from the original datasets or any neighboring dataset differing in one database record. Thus, as much as we understand the wish for overlapping $\epsilon$ parameters for the evaluated datasets, these $\epsilon$ parameters do not offer the same privacy on the evaluated datasets.}
        \item D11, W1: \textit{The experimental results on $\varphi$ are puzzling. As described in the definition of $\varphi$, when precision is below 50\%, it sounds like they "clip" it to be equal to 50\%. With this understanding, I'm puzzled by the experimental results. In Fig.~4(a), at $\eps=2$, attack precision is below 50\% and accuracy looks to be above baseline. Thus, I believe $\varphi$ should be undefined and yet it is 8.}\\
        \blue{R: We agree that this behavior is confusing. We completely revised $\varphi$ and made sure that it is well defined and returns values between 0 (min; i.e., test accuracy drops to baseline of $1/\mathbb{C}$ while MI AUC remains at original) -- 2 (max; i.e., test accuracy remains at original while MI AUC drops from $1.0$ to baseline of $0.5$).} 
        \item D12: \textit{What's up with the non-monotonicity in several Figures?}\\
        \blue{R: The observed non-monotonicity was caused by two effects. First, we did not employ early stopping in the experiments before the revision. This lead to models with very varying test accuracy at the end of the training when using DP since they are essentially already converging but following a zig-zag pattern due to perturbation. We now use early stopping to prevent such effects and have higher real world relevance. Second, for Skewed Purchases the DP perturbation is bringing the distribution of training and test data closer to each other and thus fosters generalization. This leads to increased test accuracy for some~$\epsilon$.}
        \item D13: \textit{At the end of the day, the results should carry with them a big caveat: the LDP is operating at a *much* higher $\epsilon$ than CDP. Choosing to measure privacy in terms of resistance to a specific attack could be argued as a step in the wrong direction and that $\epsilon$ is a better privacy for potential privacy loss. A benefit of the $\epsilon$-DP guarantee is that it is "future proof".}\\
       \blue{ R: We acknowledge that MIA are a more specialized threat model compared to the one considered by DP. Thus DP and MIA provide different bounds for inference risks, which we also addressed in our answer to D1. MIA can only depict a lower bound on inference risk while DP formulates an upper bound on inference risk. Our novel observation is that the bounds have a high distance for LDP which leads us to conclude that LDP with high $\epsilon$ values is still an alternative to the DP-SGD with small $\epsilon$ values. This is due to the varying neighborhood definitions of LDP and CDP.}
%        \item W2: \textit{Presentation could be improved. The abstract and introduction are poorly written. The figures are quite cluttered.}
%        \begin{itemize}
%        \end{itemize}
        \item D14, W2: \textit{The abstract/introduction has many confusing and vague phrases. Example: "we compare the privacy parameter $\epsilon$ by"}\\
        \blue{R: Thank you for pointing this out. Abstract and Introduction were rewritten.}
        \item D15, W2: \textit{The Figures are quite cluttered (e.g., showing all class sizes in all Figures, showing train and test in the same Figure).}\\
        \blue{R: We now omit the training accuracy in Fig.~(a), (e) to reduced the number of graphs from 8 to 4 s.t. they become less cluttered. Training accuracy are now provided in Table~5. The largest number of graphs contained in a Figure is now 6 (ROC curves).}
%        \item D16: \textit{Section 5 walks laboriously through each figure. Better use this space for discussion of findings.}
        \item D16: \textit{Section 5 walks laboriously through each Figure. Better use this space for discussion of findings}\\
        \blue{R: We thoroughly shortened Section~5 and instead included results on white-box MIA and extended the discussion in Section~6.}
    \end{itemize}
Reviewer 2
\vspace{1pt}
\hrule
\vspace{2pt}  
    \begin{itemize}
        \item W1: \textit{The novelty of the proposed framework is not very high. Basically an introduction of DP to the Shokri et al.~\cite{shokri2017} MI model.}\\
        \blue{R: Our work advances the state-of-the-art by a comparison of LDP and CDP mechanisms and their respective privacy parameters against membership inference attacks (MIA) to help guide data owners in choosing appropriate privacy parameters $\epsilon$. We are not aware of a study that has systematically addressed the differences between CDP and LDP for ML against MIA. Our study underpins the limited meaning of $\epsilon$ when comparing different DP mechanisms and aims to contribute to the discussion of the use of DP with meaningful privacy parameters by data scientists.}
        \item W2: \textit{The presentation needs to be improved. In particular, the proposed schemes (Figures 1 and 2) are not fully explained.}\\
        \blue{R: We incorporated your feedback and extended the descriptions of black-box and white-box MI attacks under LDP and CDP in Figure~1 and~2. The descriptions now highlight the used features, training steps and data that is exclusive to the data owner. Furthermore, they now reflect white-box and black-box MI.}
%        \item W3: \textit{Insights obtained from the experimental result is not clear.}
%        \begin{itemize}
%            \item \green{Please see our comment to D4.}
%        \end{itemize}
        \item D3: \textit{The proposed scheme (Figure~1) is an extension of the MI model~\cite{shokri2017} augmented with DP mechanisms. Assumptions and their rationale of the scheme are not explicitly presented. The adversary needs to know the (C/L)DP mechanism and $\epsilon$ to i) create the DP $shadow_i$ and ii) to perform \cali{LR}. The authors should explicitly present their assumption on the adversary's knowledge.}\\
        \blue{R: It is true that we did not explicitly state the assumptions in one section. We model an adversary who is assumed to know the utilized DP mechanism, all hyperparameters and the model structure. Indeed, we assume that the adversary to know the $\epsilon$ parameter for the DP mechanism, but not the randomness used in LDP or CDP perturbation. Both assumptions are analogous to Kerckhoff's principle in cryptography. We state the above mentioned assumptions in Section~3.}
        \item D4, W3: \textit{The experimental results for a variety of datasets are in themselves valuable. However, it is not clear what insights were obtained from the results. Is it possible to give some qualitative discussion on this result?}\\
%        \item D4: \textit{The experimental results for a variety of datasets are in themselves valuable. However, it is not clear what insights were obtained from the results. Is it possible to give some qualitative discussion on this result?}
        \blue{R: We shortened the description of the experiment section in favor of an extended discussion of experiment results. We furthermore replaced the individual discussion of MI precision and recall with an overall discussion of the area under the receiver operating curve for CDP and LDP, and analyzed a wider set of $\epsilon$ parameters to identify and present observations common to all datasets in Section~\ref{sec:phi}.}
    \end{itemize}
Reviewer 3
\vspace{1pt}
\hrule
\vspace{2pt}  
    \begin{itemize}
        \item W1: \textit{There's a lot of sloppy formatting (e.g.,author emails, oddly-sized paragraph headers). Stick with the template.}\\
        \blue{R: We apologize for the formatting issues of email addresses and paragraph headers. The paper is now in line with the VLDB template.}
        \item W2: \textit{The initial presentation of the experiments can best be described as dizzying. I'm sure the authors are concerned with space, but it would be extremely helpful for Figure captions to give more context and information about an experiment.}\\
        \blue{R: We shortened the presentation of individual experiment results in favor of extending the overall discussion. Furthermore, we extended the captions of Figures 3 -- 7 to give more context about the content. We provide more details in a technical report that provides additional graphs which do not fit into the paper length.}
        \item W3: \textit{Many of the hyperparameters and experimental details could be deferred to an online appendix to allow more space.}\\
        \blue{R: We are thankful for your suggestion to provide an online appendix. We will do so in the form of an extensive technical report on the arxiv preprint portal. The technical report will provide more experiments (e.g., effect of neural network size) and all plots (i.e., ROC curves and scatterplots for all $\mathbb{C}$ instead of only selected $\mathbb{C}$).}
        \item D1: \textit{The paper leaves me unsure if the chosen attack is suitable for evaluation. Are there stronger attacks? Is this an attack that the LDP and CDP methods are designed against? Is this an attack designed to do best against NN that use LDP/CDP methods?}\\
        \blue{R: Both, CDP and LDP limit inference on presence or absence of values or records in dataset. Membership inference attacks (MIA) target the presence or absence of a specific record in the dataset. Thus, MIA should be affected by the use of both LDP and CDP, depending on the privacy parameter $\epsilon$. Previous work by Jaymaran et al.~\cite{JE19} showed that the theoretic CDP upper bound is not reached in practice and the achievable MIA lower bound is located far apart. However, it is unclear how far apart these bounds are for LDP and this is a motivation behind our work. It is true that there is a stronger MI attack available to the black-box MI attack that was used in the original submitted paper: white-box membership inference by Nasr et al.~\cite{NSH18}. We see that white-box membership inference provides a tighter lower bound in comparison to black-box MI. In this revision we added white-box MI results in comparison to the black-box MI attack results. White-box MI, however, makes stronger assumptions on the information that is accessible by the adversary. In white-box MI the adversary is assumed to also observe the internal parameters (e.g., gradients, losses) of the neural network instead of only the outputs (e.g., labels, softmax). We observe that the MIA strength depends on the assumptions about the attacker and that white-box MI is slightly outperforming black-box MI. Per definition CDP holds for records and LDP holds for attributes. From our perspective neither definition is better or worse under MI.}
        \item D2: \textit{Using the variable $\mathbb{C}$ to refer to both the classification task and the number of classifications was a little jarring.}\\
        \blue{R: We unfortunately overloaded variable $\mathbb{C}$. At two occasions (Section~\ref{sec:experiments:texas} and~\ref{sec:experiments:purch}) we referred to $\mathbb{C}$ as the classification task, and else $\mathbb{C}$ is the number of classes. We now consistently refer to $\mathbb{C}$ as the number of distinct classes in the dataset.}
        \item D3: \textit{I'm a little confused about the dynamic number of classes, anyway -- is this just a way to add more diversity to the dataset, or do practitioners really modify the number of labels? Are the labels hierarchical, and if so, is the attack taking that into account?}\\
%        \item D2, D3: \textit{Using the variable C to refer to both the classification task and the number of classifications was a little jarring. Do practitioners modify the number of labels? Are the labels hierarchical, and if so, is the attack taking that into account?}
        \blue{R: The changes of the number of labels $\mathbb{C}$ is due to two reasons. First, for Texas Hospital Stays, Purchases and LFW the dataset consists of a large number of overall classes which contain different amounts of record, i.e.~the classes in these datasets are unbalanced. For each $\mathbb{C}$ we select the $\mathbb{C}$ classes with the largest number of records from the overall datasets for training and testing, which is in line with related work~\cite{shokri2017}. Second, for Skewed Purchases, we created a balanced data set with a fixed overall size (200,000 records) and steer number of records per class in the dataset (i.e., cluster information) by parameter $\mathbb{C}$. This fixed the overall dataset size leads to an allocation of $\frac{1}{\mathbb{C}}$ records to each class. The creation process is highlighted in Section 4 and the labels do not represent hierarchical information. We adapted our description of the methodology to clarify this aspect.}
%        \item D4: \textit{There are two models that are fully connected NN with two layers (128 x C). Isn't that just logistic regression?}
        \item D4: \textit{There are two models that are fully connected NN with two layers ($128 \times \mathbb{C}$). Isn't that just logistic regression?}\\
        \blue{R: A single layer perceptron indeed resembles logistic regression. However, there are subtle differences w.r.t.~to the used activation functions (sigmoid vs.~tanh) and the optimization mechanism (least squared error vs.~gradient descent). We thus decided to keep the neural network notation. However, we made sure to mention this aspect in the textual description of the revision.}
        \item D5: \textit{F1 and F2 could be drastically improved by making them more concrete. Show an example where I'm trying to determine if a particular image (or item) is in a dataset, and the pipeline of the undefended and defended (with LDP and CDP) approaches.}\\
%        \item D5: \textit{F1 and F2 could be drastically improved by making them more concrete. Show an example where I'm trying to determine if a particular image (or item) is in a dataset, and the pipeline of the undefended and defended (with LDP and CDP) approaches.}
        \blue{R: We generally revised Figure~\ref{fig:bb_mia} and~\ref{fig:wb_mia} to reflect data that is exclusive to the data owner and extended the description.}
        \item D6: \textit{Are precision and recall the correct measures? For example, for health data, I imagine there is a very specific rule about just "how anonymous" results need to be. In other applications, this metric could be very different. I understand the authors are using the standard metrics in the literature here, but it might be interesting to see which metrics go with which.}\\
        \blue{R: We agree that different data use cases might require different privacy measures (e.g., HIPAA requires group based measures that are in line with $k$-anonymity). Now, we compute the area under the curve of the True Positive Rate and False Positive Rate. We are convinced that this is the building block for group-based as well as for individual measures.}
        \item D7: \textit{Domain-specific measure of privacy might result in strange behavior relating the privacy parameter to the metric. For example, consider only analyzing privacy of subset of data.}\\
        \blue{R: This is a very good question. We share the view that privacy has many definitions. We consider two privacy definitions: resistance to MIA and DP. However, there are other privacy definitions which could be used to quantify privacy in machine learning (e.g., $k$-anonymity). We agree that MIA may be refined to cases where only a subset of the used training data might be sensitive and thus requires privacy protection while the rest of the training data might not require privacy. Both DP and MIA definitions can be adapted to such a requirement by adapting the DP neighboring relations and adapting the MI test data set. For MI, one could analyze a subset of training data w.r.t.~privacy-accuracy trade-off by limiting the MIA to this subset of training records and ignoring all other training records during the attack.}
    \end{itemize}
Reviewer 4
\vspace{1pt}
\hrule
\vspace{2pt}        
    \begin{itemize}
        \item W1: \textit{Not clear why central DP is being compared to LDP}\\
        \blue{R: We compare LDP and CDP, since both yield very similar protection against membership inference attacks (MIA) despite very different privacy parameters $\epsilon$. However, a discussion of just $\epsilon$ falls short w.r.t.~reflecting actual privacy protection. In contrast, if compared under a concrete attack, such as MIA, we demonstrate that high $\epsilon$ values as commonly found in LDP do not necessarily result in weak privacy, and low $\epsilon$ values such as commonly found in CDP do not imply higher privacy. We state possible advantages of LDP in our reply to W4.}
%        \item W2: \textit{Really only one DP machine learning algorithm is being evaluated (even though there are several in the literature)}
 %      \begin{itemize}
 %           \item \green{Please see our response to D3.}
 %       \end{itemize}
        \item W3: \textit{The $\epsilon$ parameters for LDP seem quite “outrageous”}\\
        \blue{R: Indeed the difference of $\epsilon$ in LDP and CDP is very large. However, this difference results from the different definitions and varying compositions for LDP and CDP. Our work demonstrates that despite the large difference in $\epsilon$ both result in similar protection against MIA at the same level of accuracy. We do not argue that either LDP or CDP is better against all possible attacks, but solely comment on MIA. This restriction is acceptable, since MIA are practical attacks with relevance to data scientists.}
        \item W4: \textit{It is not clear that the methodology used for LDP + ML even makes sense to me.}\\
        \blue{R: We are sorry for not having stated our motivation clearly enough. LDP offers a security advantage, as it allows anonymization at the data source. CDP requires continuous privacy accounting, since the original data is accessed for each training run and the privacy loss needs to continuously be updated, if multiple models are trained. Thus, an LDP protected training dataset can be used for training potentially many models with different architectures (e.g., ensemble learning), learning tasks and non-private optimizers without further need for privacy accounting. However, while it was shown that LDP comprises the same power as the statistical query model in learning theory~\cite{KLN+08}, several lower bounds for basic operations such as sums indicate that the use of LDP results in a higher worst case error compared to CDP (Beimel et al.~"Distributed private data analysis" , Chan et al.~"Optimal lower bound for differentially private multi-party aggregation"). Thus, LDP might result in lower accuracy than CDP at similar protection against MIA.}
        \item D1: \textit{I would encourage the authors to look at prior benchmark studies on ML (MLPerf~\cite{MLPERF}) or DP (e.g., Hay et al.~\cite{HAM+16}) as examples of how to set up a benchmark study. I was expecting the benchmark would study some hypothesis or questions and present findings tied to those. But I was disappointed not to find that the paper was limited to studying one question (privacy vs accuracy) across a limited set of settings.}\\
%        \item D1: \textit{Consider prior benchmark studies on ML (mlperf) or DP (e.g., Hay et al “DPBench…” SIGMOD 2016). I was disappointed not to find that the paper was limited to studying one question (privacy vs accuracy) across a limited set of settings.}
        \blue{R: Thank you for pointing out these two benchmarks. We follow all \textit{diversity of inputs principles} (i.e., different $\epsilon$ values, varying datasets scales, varying dataset size, varying dataset shape; principles 1 to 4) from DPBench, and the \textit{general rules} of MLPerf (i.e., fairness, consistent and available framework, sharing code along with this publication). However, in contrast to the two benchmarks we test the hypothesis whether LDP provides worse privacy protection than CDP due to the large differences in \eps. For this, we analyze beneficial privacy-utility trade-offs (principle 10 DPBench) in LDP and CDP. Thus we do not apply differentially private preprocessing for LDP or CDP, and do not consider adversarial side information and variability/bias of the differentially private ML models (DPBench principles 5 -- 9). We evaluate custom ML models that were used in previous work on MIA for Texas Hospital Stays and Purchases, and state-of-the-art ML Models for COLLAB and LFW. These models and data are not considered by MLPerf as benchmarks, but follow most of the training rules that are required by MLPerf.}
        \item D2: \textit{Prior empirical studies on differential privacy have not been cited: Jayaraman et al.~\cite{JE19}, Hay et al.~\cite{HAM+16}, Iyengar et al.~\cite{IST+19}.}
        \blue{R: We now cite and discuss these three works in related work.}
        \item D3, W2: \textit{I think the benchmark needs more than one CDP algorithm. First, the DP-SGD algorithm has several parameters (clipping, number of rounds, etc.), and the effect of these parameters on the datasets was not fully explored. Moreover, there are algorithms other than DP-SGD that have been proposed for learning under CDP -- empirical risk minimization (e.g., for logistic regression), PATE,\ldots which the authors have not considered.}\\
        \blue{R: It is true that we only evaluate one CDP mechanism, namely DP-SGD by Abadi et al.~\cite{abadi2016}. We chose this CDP mechanism, because we focus on central learning of a deep neural network (i.e., no federated learning and thus PATE is not applicable). Stochastic gradient descent optimizers are widely used in practice for this use case (i.e., in contrast to SGD variations found in works on DP ERM) and DP-SGD represents a direct replacement for stochastic gradient descent optimizers. We are aware that the privacy parameter $\epsilon$ and the test accuracy of the DP-SGD depends on the following, presumably complete set of parameters: clipping norm, noise multiplier, batch size, learning rate and epochs. While we do not show the experiments for variations of per parameter, the effect of each parameter on the privacy parameter $\epsilon$ is as follows~\cite{BPS19}: Greater batch sizes enhance generalization but result in greater privacy leakage, larger clipping norms result in higher privacy leakage but quicker convergence, larger numbers of epochs result in higher $\epsilon$ values, small learning rates are favorable when the batch size is small but lead to longer training and thus higher privacy parameters $\epsilon$. We optimized the parameters in our experiments to yield the best privacy-accuracy trade-off by using early stopping and thus ensuring model convergence. Approaches to DP empirical risk minimization based on output perturbation or objective function perturbation need a convex optimization function to ensure both DP and meaningful utility. Thus, the gradient optimization technique itself would be different. We leave privacy-accuracy trade-off analysis in federated learning for future work.}
        \item D4: \textit{I am not clear about why the methodology used for LDP + ML makes sense. LDP transforms the examples in the training set into a new “noisy representation” and then learns a function. Shouldn't testing work the same way -- apply randomization and then predict to get a noisy label followed by a reconstruction of the prediction?}\\
        \blue{R: This question is very important and we expanded the discussion in the revision and moved other material to an extensive technical report. For LDP a data scientist who uses perturbed training data can either validate the target model on unperturbed or perturbed test data. Here, unperturbed test data achieved better validation accuracy and thus higher utility in our experiments. 
        For black-box MIA the adversary achieves the strongest MIA accuracy if training shadow models similar to the target model, i.e., using perturbed training data and original test data. We furthermore assume the adversary to use the same DP mechanism and privacy parameter, but not the random seed that was used for perturbation by the data scientist. The adversary then has three options for learning the attack features (i.e., trained shadow model confidences on member and non-member records) after shadow model training. 
        1) Using newly perturbed training data (i.e., data with different randomness compared to shadow model training). Here, the adversary trains shadow models also on perturbed data and validates on original member and non-member records. This attack variation yielded the lowest MIA success since the adversary is essentially learning the difference between perturbed member data and unperturbed non-member data instead of original member and non-member data.
        2) Using original member data for inferring membership. Here, the adversary will learn the attack features solely on original member and non-member data. This avoids just learning the difference between two distributions (i.e., perturbed and unperturbed data). Instead the confidence difference of the trained shadow models on unperturbed member and non-member data is learned. This configuration is stated in the paper.
        3.) Using identically perturbed member data and original non-member data, i.e., assuming the adversary knows the randomness with which original member data was perturbed and thus being able to yield the same perturbed representations. Here, the adversary will learn the attack features solely on perturbed member and non-member data. This yields the highest MIA accuracy, but we dismissed this approach, since it requires access to secret information of the data analyst (i.e., the random seed).}
    \end{itemize}
}

\newpage
\twocolumn
